Adaptive Sampling for Fast Constrained Maximization of Submodular Function

Several large-scale machine learning tasks, such as data summarization, can be approached by maximizing functions that satisfy submodularity. These optimization problems often involve complex side constraints, imposed by the underlying application. In this paper, we develop an algorithm with poly-logarithmic adaptivity for non-monotone submodular maximization under general side constraints. The adaptive complexity of a problem is the minimal number of sequential rounds required to achieve the objective. Our algorithm is suitable to maximize a non-monotone submodular function under a $p$-system side constraint, and it achieves a $(p + O(\sqrt{p}))$-approximation for this problem, after only poly-logarithmic adaptive rounds and polynomial queries to the valuation oracle function. Furthermore, our algorithm achieves a $(p + O(1))$-approximation when the given side constraint is a $p$-extendible system. This algorithm yields an exponential speed-up, with respect to the adaptivity, over any other known constant-factor approximation algorithm for this problem. It also competes with previous known results in terms of the query complexity. We perform various experiments on various real-world applications. We find that, in comparison with commonly used heuristics, our algorithm performs better on these instances.

==> algorithmsLong.tex <==
\begin{algorithm2e}[t]
	\caption{\rndseq{}$(X, S, \ind{})$}
	\label{alg:rndseq}
	\begin{algorithmic}[1]
	    \STATE $A \gets \emptyset$;
 	    \WHILE{$X \neq \emptyset $}\label{alg:beginWhileAlg3}
 	    \STATE sort the points $\{x_i\}_i = X$ randomly;
 	    \STATE $\eta \gets \max \{ j \colon S \cup A \cup \{x_i\}_{i \leq j} \in \ind{} \} $;
 	    \STATE $A \gets A \cup \{x_1, \dots,x_{\eta}\}$;\label{alg:sequence:alg}
 	    \STATE $X \gets \{e \in X\setminus (S \cup A) \colon S \cup A \cup e  \in \ind{} \}$;\label{alg:rndseq:Y1}
        \ENDWHILE \label{alg:endWhileAlg3}
   	\STATE \textbf{return} $A$;
   	\end{algorithmic}
\end{algorithm2e}
\begin{algorithm2e}[t]
	\caption{\asplusplus{}$(f, V, \ind{},\lambda, \varepsilon)$.// input has changed (???) describe parameters in lemmas}
	\label{alg:samplplusplus}
	\begin{algorithmic}[1]
	\STATE $S \gets \emptyset$;
	\STATE $X \gets \argmax_e \{ f(e) \colon e \in V \land e \in \ind \}$;
	\STATE $\delta \gets f(X)$, $\delta_0 \gets \lambda f(X) $;
	\WHILE{$\delta \geq \delta_0$}\label{alg:samplplusplus:beginWhile1}
   \WHILE {$X \neq \emptyset$}\label{alg:sampl:beginWhile2}
    \STATE $\{a_j\}_{j\in J } \gets \mbox{\rndseq{}}(X,S,\ind{})$;\label{alg:sampl:binaryBegin}
    \STATE $J \gets \mbox{\geometric}(1, \absl{J}, 1 - \varepsilon)$; // explain this step
    \STATE $\eta \gets \mbox{\binarysearch}(J, \max \{j \in J \colon \absl{X_j} > (1 - \varepsilon ) \absl{X} \})$ with $X_j = \{e \in X \colon f (e \mid S \cup \{a_1, \dots, a_j \} ) \geq \delta \land S \cup \{a_1, \dots, a_j \} \cup e \in \ind \}$
   	\STATE $A \gets \mbox{\unif}(\{a_1, \dots, a_{\eta}\}, \boldsymbol\varphi_1)$;
    \STATE $X \gets X_{\eta}$; $S \gets S \cup A $;
    \ENDWHILE \label{alg:sampl:endWhile2} 
    \STATE $\delta \gets ( 1 - \varepsilon )\delta$;
    \STATE $X \gets \{e \in V \colon f(e\mid S) \geq \delta \land S \cup e \in \ind  \}$;\label{alg:sampl:defX}
    \ENDFOR \label{alg:samplplusplus:endWhile1}
   	\STATE \textbf{return} $S$;
   	\end{algorithmic}
\end{algorithm2e}

==> algorithmsShort.tex <==
\begin{algorithm2e}[t]
	\caption{\kas{}$(f, V, \ind{}, \varepsilon, p,q,m)$}
	\label{alg:ksampl}
	\begin{algorithmic}[1]
	\STATE $\lambda \gets \varepsilon (p + 1)/r $;
	\FOR{$j \leq m$ iterations} \label{for:kas_begin}
    {
        \STATE $\Omega_j \gets \asplusplus{}(f, V, \ind{}, \delta_0, \varepsilon)$;\label{for:kas_line1}
        \STATE $\Lambda_j \gets \mbox{\unif} (\Omega_j, q)$;\label{alg:k-sampl_random}
        \STATE $V \gets V \setminus \Omega_j$;
   	}
   	\ENDFOR  \label{for:kas_end}
   	\STATE \textbf{return} $\argmax_j \{f(\Omega_j), f(\Lambda_j) \}$\;
   	\end{algorithmic}
\end{algorithm2e}

==> tables.tex <==

\colorlet{tablecolor}{black!10}
\renewcommand{\arraystretch}{1.35}%1.35
\begin{table}[h]
\center
\begin{tabular}{cc|c|cc|cc|}
\cline{2-7}
& \multicolumn{1}{|c|}{\fantom{}} & \greedy{} & \multicolumn{2}{c}{\kas{}} & \multicolumn{2}{|c|}{\random{}} \\
\cline{4-7}
& \multicolumn{1}{|c|}{} &           & mean & s.d.                 & mean & $\ \ \ $s.d.$\ \ \ $                    \\
\hline
\rowcolor{tablecolor} \multicolumn{1}{|c|}{movie (1)} & 21.1636 & 20.7486 & 22.3783 & 0.340616  & 15.1944 & 1.47299  \\
 \multicolumn{1}{|c|}{movie (2)} & 17.2829 & 17.2829 & 17.9722 & 0.325992  & 12.5095 & 1.17141  \\
\rowcolor{tablecolor} \multicolumn{1}{|c|}{movie (3)} & 17.344  & 15.986  & 16.1478 & 0.475222  & 12.2402 & 1.26988  \\
 \multicolumn{1}{|c|}{movie (4)} & 12.377  & 12.377  & 12.1912 & 0.119175  & 9.50488 & 0.868505 \\
\rowcolor{tablecolor} \multicolumn{1}{|c|}{movie (5)} & 16.2405 & 16.2405 & 17.3745 & 0.265393  & 11.6482 & 1.03631  \\
 \multicolumn{1}{|c|}{movie (6)} & 14.217  & 14.217  & 13.8881 & 0.222973  & 10.2279 & 0.944217 \\
\rowcolor{tablecolor} \multicolumn{1}{|c|}{movie (7)} & 8.3842  & 8.41786 & 7.55106 & 7.10543e-15 & 7.07657 & 0.587772 \\
 \multicolumn{1}{|c|}{movie (8)} & 14.5017 & 14.3214 & 14.604  & 0.27744   & 10.9951 & 1.10049  \\
\rowcolor{tablecolor} \multicolumn{1}{|c|}{movie (9)} & 21.9102 & 21.8762 & 21.7451 & 0.565241  & 14.0454 & 1.56799  \\
 \multicolumn{1}{|c|}{movie (10)} & 10.6722 & 10.6722 & 11.473  & 8.88178e-15 & 9.4753  & 0.5978 \\
\rowcolor{tablecolor} \multicolumn{1}{|c|}{movie (11)} & 18.9345 & 18.823  & 20.0142 & 0.477174  & 14.3845 & 1.20575  \\
 \multicolumn{1}{|c|}{movie (12)} & 14.2948 & 14.1852 & 14.3486 & 0.0736    & 10.8111 & 0.908946 \\
\rowcolor{tablecolor} \multicolumn{1}{|c|}{movie (13)} & 13.4546 & 13.4546 & 13.1502 & 0.107649  & 10.062  & 0.972653 \\
 \multicolumn{1}{|c|}{movie (14)} & 15.3864 & 15.1939 & 15.1143 & 0.0840961 & 11.7023 & 1.00893  \\
\rowcolor{tablecolor} \multicolumn{1}{|c|}{movie (15)} & 18.0012 & 17.5787 & 18.6568 & 0.15169   & 14.2627 & 1.16388  \\
 \multicolumn{1}{|c|}{movie (16)} & 14.8608 & 13.8455 & 15.2768 & 0.346216  & 11.7006 & 1.05791  \\
\rowcolor{tablecolor} \multicolumn{1}{|c|}{movie (17)} & 20.5922 & 20.5922 & 19.9888 & 0.307146  & 13.5201 & 1.25515  \\
 \multicolumn{1}{|c|}{movie (18)} & 19.2075 & 19.2075 & 19.5614 & 0.374759  & 12.5197 & 1.17543  \\
\rowcolor{tablecolor} \multicolumn{1}{|c|}{movie (19)} & 18.3385 & 18.3661 & 18.7087 & 0.211137  & 13.1053 & 1.15827  \\
 \multicolumn{1}{|c|}{movie (20)} & 16.0257 & 16.0257 & 16.1194 & 0.231575  & 11.3701 & 1.14547  \\
\rowcolor{tablecolor} \multicolumn{1}{|c|}{movie (21)} & 15.185  & 14.9873 & 15.7315 & 0.26301   & 11.7207 & 1.06622  \\
\hline
\end{tabular}
\caption{Solution quality for the experiments on Video Summarization, as described in Section \ref{section:DPP}. Ranks displayed in Figure \ref{fig:1a} are based on these results. Note that the results for the \kas{} on movie (7) and movie (10) exhibit little variance, in comparison with the other result. This is probably due to the large number of side constraints and a large parameter $\Delta$.}
\label{table1}
\end{table}
%
%
\begin{table}
\center
\begin{tabular}{cc|c|cc|cc|}
\cline{2-7}
& \multicolumn{1}{|c|}{\fantom{}} & \greedy{} & \multicolumn{2}{c}{\kas{}} & \multicolumn{2}{|c|}{\random{}} \\
\cline{4-7}
& \multicolumn{1}{|c|}{} &           & mean & s.d.                 & mean & $\ \ \ $s.d.$\ \ \ $                    \\
\hline
\rowcolor{tablecolor} \multicolumn{1}{|c|}{movie (1)} & 85 & 15 & 13.28 & 0.938936  & 15.38 & 0.505569 \\
\multicolumn{1}{|c|}{movie (2)} & 76 & 14 & 12.91 & 0.426497  & 14.46 & 0.590254 \\
\rowcolor{tablecolor} \multicolumn{1}{|c|}{movie (3)} & 68 & 12 & 10.84 & 0.417612  & 13.97 & 0.727393 \\
\multicolumn{1}{|c|}{movie (4)} & 58 & 10 & 11.86 & 0.510294  & 12.21 & 0.697065 \\
\rowcolor{tablecolor} \multicolumn{1}{|c|}{movie (5)} & 73 & 13 & 13.22 & 0.878408  & 14.09 & 0.664756 \\
\multicolumn{1}{|c|}{movie (6)} & 68 & 12 & 11.47 & 0.767529  & 13.15 & 0.71239  \\
\rowcolor{tablecolor} \multicolumn{1}{|c|}{movie (7)} & 39 & 8  & 7     & 0         & 8.83  & 0.693614 \\
\multicolumn{1}{|c|}{movie (8)} & 67 & 12 & 9.98  & 0.423792  & 13    & 0.748331 \\
\rowcolor{tablecolor} \multicolumn{1}{|c|}{movie (9)} & 87 & 15 & 12.72 & 0.762627  & 15.41 & 0.567362 \\
\multicolumn{1}{|c|}{movie (10)} & 41 & 9  & 9     & 0         & 9.56  & 0.621611 \\
\rowcolor{tablecolor} \multicolumn{1}{|c|}{movie (11)} & 76 & 15 & 13.06 & 0.562494  & 14.61 & 0.760197 \\
\multicolumn{1}{|c|}{movie (12)} & 63 & 11 & 10.12 & 0.40694   & 12.53 & 0.767529 \\
\rowcolor{tablecolor} \multicolumn{1}{|c|}{movie (13)} & 72 & 13 & 11.65 & 0.47697   & 12.98 & 0.647765 \\
\multicolumn{1}{|c|}{movie (14)} & 51 & 11 & 10.01 & 0.0994987 & 11.83 & 0.584038 \\
\rowcolor{tablecolor} \multicolumn{1}{|c|}{movie (15)} & 71 & 14 & 11.78 & 0.878408  & 14.81 & 0.643351 \\
\multicolumn{1}{|c|}{movie (16)} & 61 & 12 & 11.03 & 0.298496  & 12.82 & 0.792212 \\
\rowcolor{tablecolor} \multicolumn{1}{|c|}{movie (17)} & 81 & 14 & 11.86 & 0.616766  & 14.76 & 0.649923 \\
\multicolumn{1}{|c|}{movie (18)} & 78 & 14 & 12.61 & 0.733417  & 14.82 & 0.683813 \\
\rowcolor{tablecolor} \multicolumn{1}{|c|}{movie (19)} & 70 & 14 & 11.58 & 1.03131   & 14.24 & 0.69455  \\
\multicolumn{1}{|c|}{movie (20)} & 66 & 11 & 10.96 & 0.760526  & 13.55 & 0.698212 \\
\rowcolor{tablecolor} \multicolumn{1}{|c|}{movie (21)} & 68 & 14 & 11.68 & 0.614492  & 13.67 & 0.749066  \\
\hline
\end{tabular}
\caption{Run time, in terms of adaptive rounds, for the experiments on Video Summarization, as described in Section \ref{section:DPP}. Ranks displayed in Figure \ref{fig:1b} are based on these results. Note that the results for the \kas{} on movie (7) and movie (10) exhibit no variance. This is probably due to the large number of side constraints and a large parameter $\Delta$.}
\label{table2}
%
%
%
\bigskip
\bigskip
\bigskip
\begin{tabular}{|c|c|}
\hline
movie (1) & \cellcolor{tablecolor} Along Came Polly    \\
movie (2)                                   & American Wedding  \\
movie (3) & \cellcolor{tablecolor} Basic Instinct           \\
movie (4)                                   & Battle Cry                \\
movie (5) & \cellcolor{tablecolor} Casino Royale         \\
movie (6)                                   & 2 Fast 2 Furious      \\
movie (7) & \cellcolor{tablecolor} Funny Girl                \\
\hline
\end{tabular}
\begin{tabular}{|c|c|}
\hline
movie (8)  & \cellcolor{tablecolor} Giant         \\
movie (9)                        & Hitch   \\
movie (10) & \cellcolor{tablecolor} Irma la Douce         \\
movie (11)                       & The Italian Job    \\
movie (12) & \cellcolor{tablecolor} Million Dollar Baby     \\
movie (13)                       & Monster-in-Law        \\
movie (14) & \cellcolor{tablecolor} Mr. \& Mrs. Smith \\
\hline
\end{tabular}
\begin{tabular}{|c|c|}
\hline
movie (15) & \cellcolor{tablecolor} National Treasure      \\
movie (16)                       & Ocean’s Eleven         \\
movie (17) & \cellcolor{tablecolor} Twelve O’Clock High    \\
movie (18)                       & The Princess Diaries 2 \\
movie (19) & \cellcolor{tablecolor} Schindler’s List       \\
movie (20)                       & The Ten Commandments   \\
movie (21) & \cellcolor{tablecolor} The Departed           \\
\hline
\end{tabular}
\caption{List of movies to perform the experiments on Video Summarization as described in Section \ref{section:DPP}. Each dataset is taken from the FLIC repository \cite{modec13}, and it consists of $200$ snapshots. We choose these movies, based on the number of available snapshots.}
\label{table3}
\end{table}

